Adaptive Address Family Selection for Latency-Sensitive Applications on Dual-stack Hosts

Latency is becoming a key factor of performance for Internet applications and has triggered a number of changes in its protocols. Our work revisits the impact on latency of address family selection in dual-stack hosts. Through RIPE Atlas measurements, we analyse the address families latency difference and establish two requirements based on our findings for a latency-focused selection mechanism. First, the address family should be chosen per destination. Second, the choice should be able to evolve over time dynamically. We propose and implement a solution formulated as an online learning problem balancing exploration and exploitation. We validate our solution in simulations based on RIPE Atlas measurements, implement and evaluate our prototype in four access networks using Chrome and popular web services. We demonstrate the ability of our solution to converge towards the lowest-latency address family and improve the latency of transport connections used by applications.

==> e2e-latency-popular.tex <==
Popular Internet services are structured differently than RIPE anchors. While anchors are single machines to which a transport connection can be established directly, popular services often have distributed infrastructures in several locations and place their servers behind load-balancers that can terminate the transport connections close to the users. We argue that measuring the end-to-end latency in this context is relevant as it brings a different kind of destinations into perspective.

We reuse the RIPE probes as our measurement vantage point and leverage the RIPE Ping test to measure the end-to-end latency towards these services\footnote{We will provide links towards all public measurements presented in this section in the camera-ready version of this work.}. Using the RIPE HTTP test poses some issues as the size of HTTP responses is not controlled anymore. It is very likely to vary between services and could overload some probes. We choose to request 5 ping packets per measurement and select the median RTT as the measurement result. We force each probe to do the DNS resolution of the service domain name before pinging the resolved address to better represent the latency experienced by users in these networks when sending packets to these services.

To find popular services, we use the Tranco list~\cite{LePochat2019} generated on the \nth{5} of April 2023\footnote{Available at \url{https://tranco-list.eu/list/6JL4X}} and choose the top 20 domain names for which an IPv4 and IPv6 address can be resolved from our campus network. The resulting list has a diversity of companies and organisations providing popular services to a significant part of the Internet users. We only consider the top 20 domain names to fit within the rate limits defined by the RIPE Atlas platform~\cite{ripe-atlas-limits}.


\textbf{Distribution of IPv4 and IPv6 request completion times}. We selected 1000 probes, i.e. the maximum number of RIPE probes that can be selected for a measurement~\cite{ripe-atlas-limits}, from the dual-stack probes connected on the \nth{12} April of 2023 and ran IPv4 and IPv6 pings towards the top 20 domain names, repeating the measurements 12 hours later. 945 probes took part in the measurements and 930 probes reported a total of \numprint{51750} results.\todo[inline]{This is way lower than the expected $930*20*2*2 = 74400$ amount of tests} When filtering out median RTT values within the \nth{5} or \nth{95} percentiles and pairing the results to compute IPv4/IPv6 median RTT ratios towards a destination, we obtain \numprint{19244} ratios.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/ripe_ping_ratio_tranco_12_apr_2023.pdf}
    \caption{Distribution of IPv4/IPv6 pings median RTT from RIPE probes to the Tranco top 20 domain names on the \nth{12} of April 2023.}
    \label{fig:ripe-ping-ratio-tranco-dh}
\end{figure}

\figurename~\ref{fig:ripe-ping-ratio-tranco-dh} reports the distribution of these ratios. This distribution has two differences compared to the ratios of HTTP requests completion times between probes and anchors. First, there is more variance in the distribution with less points in the central region. Second, IPv4 has a lower median ping RTT than IPv6 in $60\%$ of the comparisons. \textbf{When considering popular services, the latency diversity between IPv4 and IPv6 increases and IPv4 is slightly favored}.

\textbf{Proportion of destinations reached with the best path}. We then analyse how this diversity is spread among probes by computing the percentage of destinations that can be reached with the lowest median ping RTT using the best performing path on average for each probe. We use the same definition of best performing path as in Section~\ref{sec:e2e-latency-general-dh}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/ripe_ping_best_path_12_apr_2023.pdf}
    \caption{Distribution of the percentage of destinations for each probe that can be reached with the lowest HTTP request completion time based on the best performing path on average on the \nth{12} of April 2023.}
    \label{fig:ripe-ping-best-path-tranco-dh}
\end{figure}

\figurename~\ref{fig:ripe-ping-best-path-tranco-dh} reports the distribution of this percentage for all 930 participating probes in our measurements. We can observe that it is similar to the distribution towards RIPE anchors. \textbf{Most dual-stack probes must use both address families to reach all popular services with the lowest latency.}





